Convolutional Learning on Multigraphs

Graph convolutional learning has led to many exciting discoveries in diverse areas. However, in some applications, traditional graphs are insufficient to capture the structure and intricacies of the data. In such scenarios, multigraphs arise naturally as discrete structures in which complex dynamics can be embedded. In this paper, we develop convolutional information processing on multigraphs and introduce convolutional multigraph neural networks (MGNNs). To capture the complex dynamics of information diffusion within and across each of the multigraph's classes of edges, we formalize a convolutional signal processing model, defining the notions of signals, filtering, and frequency representations on multigraphs. Leveraging this model, we develop a multigraph learning architecture, including a sampling procedure to reduce computational complexity. The introduced architecture is applied towards optimal wireless resource allocation and a hate speech localization task, offering improved performance over traditional graph neural networks.

==> v10/sec_discussion.tex <==
%!TEX root = ../compiler_paper.tex







%%----------------------------------------------------------------------------------
%%---------------- SECTION: DISCUSSION--------------------------------
%%----------------------------------------------------------------------------------
%
\section{Discussion}\label{sec:discussion}

The notion of stability stated in Definition~(\ref{def:stabilityoperators1}) is expressed in terms of the size of the deformation $\bbT(\bbS)$, and Theorem~\ref{theorem:HvsFrechet} states that the size of $\bbT(\bbS)$ is bounded by the norm of the Fr\'echet derivative of the filters acting on $\bbT(\bbS)$, and this is true for any arbitrary perturbation $\bbT(\bbS)$ indicated in eqn.~(\ref{eqn_def_perturbation_model_20}). This last attribute allowed to find that the stability of AlgNN is independent of the commutativity of the algebra and the commutativity of the shift operators with respect to $\bbT(\bbS)$. This is consistent with the first stability results found in~\cite{parada_algnn} but the bounds obtained are tighter since the non commutativity between $\bbS$ and $\bbT(\bbS)$ in~\cite{parada_algnn} affected the constants in the stability bounds.

To guarantee stability, the functional complexity of the deformation $\bbT(\bbS)$ is processed by the operator $\bbD_{p}(\bbS)$ imposing restrictions on $p(\bbS)$ and therefore affecting its selectivity. However, the properties of the maps $\sigma_{\ell}$ between layers allow the redistribution of the frequency content. It is worth pointing out that the, unlike in commutative algebras, frequencies are not necessarily associated to scalar values, however we know this redistribution occurs since the nonlinearities $\eta_{\ell}$ preserve the energy of the signal. This tradeoff between stability and selectivity is partly associated to the Lipschitz constants $L_{0}$ and $L_{1}$.










==> v10/sec_filters_MSP.tex <==
%!TEX root = ../compiler_paper.tex





%%---------------------------------
%%------------ Sub-Section ----------
%%---------------------------------

\subsection{Filters and Convolutions on Multigraphs} 

 In this section, we introduce multigraph filters and convolutions. The notion of filtering and convolution in multigraphs can be derived naturally from algebraic signal processing (ASP) when considering polynomial algebras with multiple generators.

%%------------------------------------------------------
%%-------------------- DEFINITION  -----------------------
%%------------------------------------------------------

\begin{definition}
	Let $M= \left( \ccalV, \{ \ccalE \}_{g=1}^{m}  \right)$ be a multigraph with shift operators $q_{\boldsymbol{a},k}$. Given coefficients $h_{\boldsymbol{a},k}$, a multigraph filter defined as: 
	
	\begin{equation}
    \mathbf{H}(\mathbf{S}_1, \dots, \mathbf{S}_m) = \sum_{k=0}^\infty \sum_{\boldsymbol{a}\in \Omega_{k}} h_{\boldsymbol{a},k}q_{\boldsymbol{a},k}(\mathbf{S}_1, \dots, \mathbf{S}_m).
\end{equation}
\end{definition}

%%----------------- End of Definition  ----------------------

Notice that no assumption has been made about the commutativity of the underlying graph shift operators $\{ \bbS_\ell \}_{\ell=1}^{m}$. The composition of the action of two filters $\mathbf{H}_1$ and $\mathbf{H}_2$ is naturally defined by the product of polynomials $\mathbf{H}_1\mathbf{H}_2$, and the operations of addition and multiplication by scalars also follow from the traditional version of these operations with polynomials. As we will show in the next section, this is a consequence of the fact that the set of multigraph filters is a homeomorphic image of a polynomial algebra on a space of matrices.

Without commutativity, we cannot take for granted the shift invariance property associated to graph filters. We state formally shift invariance for multigraph filters in the following definition.



%%------------------------------------------------------
%%-------------------- DEFINITION  -----------------------
%%------------------------------------------------------

\begin{definition}
	Let $\mathbf{H}(\bbS_1, \ldots, \bbS_m)$ be a multigraph filter on $M= \left( \ccalV, \{ \ccalE \}_{\ell=1}^{m}  \right)$ with shift operators $q_{\boldsymbol{a},k}$. Then, we say that $\mathbf{H}$ is shift invariant with respect to $q_{\boldsymbol{a},k}$ if
	%
	%
	%
	\begin{equation}
	q_{\boldsymbol{a},k}   \mathbf{H}(\bbS_1, \ldots, \bbS_m)
	=
	\mathbf{H}(\bbS_1, \ldots, \bbS_m) q_{\boldsymbol{a},k}
	.
	\end{equation}
	%
	%
	%
\end{definition}

%%----------------- End of Definition ------------------------

We can see that when we have commutative shift operators, shift invariance is guaranteed. Some families of filters could have shift invariance with respect to only specific shift operators.

%%------------------------------------------
%%-------------- LEMMA -------------------
%%------------------------------------------

\begin{lemma}
	Let $M= \left( \ccalV, \{ \ccalE \}_{\ell=1}^{m}  \right)$ be a multigraph with shift operators $q_{\boldsymbol{a},k}$. If $\bbS_i \bbS_j = \bbS_j \bbS_i$ for all $i,j$, then any multigraph filter $\mathbf{H}(\bbS_1, \ldots, \bbS_m)$ on $M$ is shift invariant with respect to any $q_{\boldsymbol{a},k}$.
\end{lemma}

%%------------ End of LEMMA --------------

\begin{example}
	\blue{Family of filters with specific invariance respect to a particular shift operator}
\end{example}


\begin{example}
		\blue{content}
\end{example}


The result of applying the multigraph filter $\mathbf{H}(\mathbf{S}_1, \dots, \mathbf{S}_M)$ to a signal $\bbx$ is a new signal $\bbz$ given by:

	\begin{equation}
    \bbz = \mathbf{H}(\mathbf{S}_1, \dots, \mathbf{S}_M)\bbx = \sum_{k=0}^K \sum_{\boldsymbol{a}\in \Omega_{k}} h_{\boldsymbol{a},k}q_{\boldsymbol{a},k}(\mathbf{S}_1, \dots, \mathbf{S}_M)\bbx.
\end{equation}


This operation $\bbz = \mathbf{h} \ast_{q_{\boldsymbol{a},k}} \bbx$ is the \emph{multigraph convolution} of the filter $\mathbf{h} = \{h_{\boldsymbol{a},k}\}$ with the signal $\bbx$.
 



















==> v10/sec_stability_multigraph_nn.tex <==
%!TEX root =../compiler_paper.tex
%!TEX root =../compiler_paper.tex





%%---------------------------------------------------------------
%%-------- SECTION: STABILITY IN MULTIGRAPH NEURAL NETWORKS ----------
%%---------------------------------------------------------------

\section{Stability of Multigraph Neural Networks}




\blue{
	------
	Here we show the stability results expressing each polynomial as the sum of polynomials of a single variable plus polynomials of mixed terms. We can show how when the multigraph provides little to no information extra to individual graphs, it leads to large errors in the presence of perturbations in the shift operators.
	------\\
	We can be also more specific about the stability bounds, making emphasis to the particular type of non linearities that we used in the simulations.
	}













